Multimodal Meta-Learning for Time Series Regression

Recent work has shown the efficiency of deep learning models such as Fully Convolutional Networks (FCN) or Recurrent Neural Networks (RNN) to deal with Time Series Regression (TSR) problems. These models sometimes need a lot of data to be able to generalize, yet the time series are sometimes not long enough to be able to learn patterns. Therefore, it is important to make use of information across time series to improve learning. In this paper, we will explore the idea of using meta-learning for quickly adapting model parameters to new short-history time series by modifying the original idea of Model Agnostic Meta-Learning (MAML) \cite{finn2017model}. Moreover, based on prior work on multimodal MAML \cite{vuorio2019multimodal}, we propose a method for conditioning parameters of the model through an auxiliary network that encodes global information of the time series to extract meta-features. Finally, we apply the data to time series of different domains, such as pollution measurements, heart-rate sensors, and electrical battery data. We show empirically that our proposed meta-learning method learns TSR with few data fast and outperforms the baselines in 9 of 12 experiments.

==> atexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> support.tex <==
\begin{document}


\section{Data pre-processing}


\label{section:data-preprocessing}

In this section, we introduce the different pre-processing steps done for training the different models. It is important to note that we split the datasets in meta-training, meta-validation and meta-testing. To train the models that are not originally suited for a meta-training procedure, we create two additional datasets: training and validation. The meta-training and training datasets come from the same source TSR task, the difference is that we apply the algorithm \ref{alg:meta-windows_generation} to generate the meta-training dataset, whereas we just apply the rolling window $\mathcal{W}_{\delta, k}(\cdot)$  to generate the training dataset. Said that, a group comprising five different datasets is generated (meta-training, training, meta-validation, validation and meta-testing).

In general, we apply the following steps to each original dataset in order to generate the group of datasets, although some of them may be exempt of one or more:

\begin{itemize}
    \item \textbf{Manual feature selection}: it means, to access the feature that we are going to use according to expert knowledge or some other criteria.
    \item \textbf{Dataset splitting}: to determine which time series are going to be held for training (or meta-training), validation (or meta-validation) and meta-testing. The following steps are applied to every split dataset, by having into account that any pre-processing parameter (such as the mean for imputation or the standard deviation for the standardization) are only computed on the training dataset.
    \item \textbf{Imputation}: to eliminate the not-valid values by replacing them with the mean or some other reasonable value.
    \item \textbf{Feature engineering}: to transform existing features or to create new features.
    \item \textbf{Target engineering}: to transform or create a target variable.
    \item \textbf{Standardization}: to standardize the features by subtracting the mean and dividing by the standard deviation plus a min-max normalization of the target variable so that it remains between 0 and 1.
    \item \textbf{Rolling window}: to divide the time series in chunks called windows by applying the process explain in section \ref{section:meta-windows}. The parameters of the rolling window, window size and step size, should be carefully set, as they trades off the diversity of samples within the respective meta-window and the number of total possible meta-windows. As explained previously, the tasks in meta-learning must be diverse and there should be many of them. In our context, it refers to the virtual tasks or, more precisely, to the meta-windows. Due to the nature of the problem, time series, it is possible to notice that meta-windows with a small step-size will have less diversity as the samples are more (temporally) correlated. On the other hand, having bigger step-sizes will decrease the total number of meta-windows, and hence, the available number of virtual tasks.
    
    \item \textbf{Meta-windows generation}: to generate the meta-windows by applying the algorithm \ref{alg:meta-windows_generation}. This is only applied if the dataset is applied for the assessment on test (meta-testing) or if it use for training and validation on MAML or MMAML (meta-training and meta-validation).
\end{itemize}

In the following sections, it will be explained in more detailed how every step is carried out for every specific dataset.

\subsection{Air Pollution Dataset Pre-processing}

The list of variables selected as features are (citing the original name): \textit{ month, data, hour, season, DEWP, HUMI, PRES, TEMP, cbwd, Iws, precipitation, Iprec}. The target is set to be the last recorded value of \textit{PM US Post} for a given window. We included all possible variables, only discarding \textit{year}, because this could make the dataset prone to memorization overfitting. Given that we have five different cities (five files), we decided to assign every file to a type of dataset as shown in table \ref{table:pollution_split}. This decision is arbitrary and there is no specific reason for this choice. Any other assignation would be equally valid. 

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|cl}
\cline{1-3}
\textbf{City} & \textbf{Data size} & \textbf{Meta-set}                  & \textbf{} &  \\ \cline{1-3}
Beijing       & 52584              & \cellcolor[HTML]{FFCE93}Meta-train &           &  \\ \cline{1-3}
Chengdu       & 52584              & \cellcolor[HTML]{FFCE93}Meta-train &           &  \\ \cline{1-3}
Guangzhou     & 52584              & \cellcolor[HTML]{FFCE93}Meta-train &           &  \\ \cline{1-3}
Shanghai      & 52584              & \cellcolor[HTML]{AFD095}Meta-val   &           &  \\ \cline{1-3}
Shenyang      & 52584              & \cellcolor[HTML]{D4D7F5}Meta-test  &           &  \\ \cline{1-3}
\textbf{Total}         & \textbf{262920}             & \textbf{Total Dataset}                      &           &  \\ \cline{1-3}

\end{tabular}
\caption{Air Pollution Dataset Split}
\label{table:pollution_split}
\end{table}

To impute the values, the target is set to zero in case of not-valid numbers (NA). In case of numerical features, the NAs are replace by the interpolated values. The wind direction (\textit{cbwd}) is converted from category to numbers by mapping it values to numbers in the range 0-4. The invalid values for \textit{precipitation} and \textit{Iprec} are set to -1, as they have numerical values but with categorical semantics, therefore making up a new category. The total number of channels is 14, where every the frequency is a sample every hour.

This dataset did not need any special further feature or target engineering. After standardization, the parameters for the rolling window; namely the window size and step size, must be carefully set. The window size is chosen equal to 5, following \cite{ma2019air} and \cite{iskandaryan2020air}. The figure \ref{fig:acorr_pollution} shows the auto-correlation plot of the target variable, which is a proxy of how similar are the windows with respect to other ones. As it depicts, setting the step size to 1 is a good decision, as the targets are not so correlated in comparison to the behaviour exhibited on the other two datasets and it does not compromise the number of possible virtual tasks.

\begin{figure} [H]
\centering
\includegraphics[width=6cm]{supplementary-images/acorr_pollution.pdf}
\caption{Auto-correlation of the target in Pollution Dataset.}
\label{fig:acorr_pollution}
\end{figure}

\subsection{Heart-rate Dataset Pre-processing}


This dataset requires more pre-processing, since the signals are sampled at different frequencies. We select 13 signals: 3 accelerometer signals from the chest (\textit{chest-ACC, chest-ACC1, chest-ACC2} - 700 Hz), from the wrist (\textit{Wrist-ACC, wrist-ACC1, wrist-ACC2} - 32 Hz), temperature from the chest and wrist (\textit{chest-temp, wrist-temp} - 4 Hz), electro-dermal activity from the chest and wrist (\textit{chest-EDA, wrist-EDA} - 4 Hz), electromiography from the chest (EMG - 700 Hz), respiratory sensor (Resp - 700 Hz) and photoplethysmography (PPG - 64 Hz). A total of 13 signals are used. Since they have different sampling frequency, we decide to reduce all the signals into a 4 Hz frequency. Hence, all the signals whose frequency were greater than 4 Hz where aggregated (or filtered, in signal processing terminology) accordingly. 

The target is taken from the ECG signal from the chest sensor (700 Hz). Since every sample corresponds to a quarter of a second (because of 4 Hz sampling frequency), in order to compute the ground truth for the heart rate we count how many peaks occur in a window of 175 samples (700/4), as the original frequency is 700 Hz, and take the average of this number (so-called instantaneous heart-rate) within the window. No imputation was needed for features and the target. There were 15 subjects records, which were split in meta-datasets as described on table \ref{table:hear_rate_split}.

\begin{table}[]
\centering
\begin{tabular}{|c|c|c|ll}
\cline{1-3}
\textbf{Subject} & \textbf{Data size} & \textbf{Meta-set} & \multicolumn{1}{c}{\textbf{}} &  \\ \cline{1-3}
S1               & 36815              & \cellcolor[HTML]{FFCE93}Meta-train        & \multicolumn{1}{c}{}          &  \\ \cline{1-3}
S2               & 32788              & \cellcolor[HTML]{FFCE93}Meta-train        & \multicolumn{1}{c}{}          &  \\ \cline{1-3}
S3               & 34931              & \cellcolor[HTML]{FFCE93}Meta-train        & \multicolumn{1}{c}{}          &  \\ \cline{1-3}
S4               & 36567              & \cellcolor[HTML]{FFCE93}Meta-train        & \multicolumn{1}{c}{}          &  \\ \cline{1-3}
S5               & 37188              & \cellcolor[HTML]{FFCE93}Meta-train        & \multicolumn{1}{c}{}          &  \\ \cline{1-3}
S6               & 20967              & \cellcolor[HTML]{FFCE93}Meta-train        & \multicolumn{1}{c}{}          &  \\ \cline{1-3}
S7               & 37338              & \cellcolor[HTML]{FFCE93}Meta-train        &                               &  \\ \cline{1-3}
S8               & 32286              & \cellcolor[HTML]{FFCE93}Meta-train        &                               &  \\ \cline{1-3}
S9               & 34208              & \cellcolor[HTML]{FFCE93}Meta-train        &                               &  \\ \cline{1-3}
S10              & 42559              & \cellcolor[HTML]{AFD095}Meta-val          &                               &  \\ \cline{1-3}
S11              & 36160              & \cellcolor[HTML]{AFD095}Meta-val          &                               &  \\ \cline{1-3}
S12              & 31623              & \cellcolor[HTML]{AFD095}Meta-val          &                               &  \\ \cline{1-3}
S13              & 36511              & \cellcolor[HTML]{D4D7F5}Meta-test         &                               &  \\ \cline{1-3}
S14              & 35798              & \cellcolor[HTML]{D4D7F5}Meta-test         &                               &  \\ \cline{1-3}
S15              & 31724              & \cellcolor[HTML]{D4D7F5}Meta-test         &                               &  \\ \cline{1-3}
\textbf{Total}            & \textbf{517463}             & \textbf{Total data-set}    &                               &  \\ \cline{1-3}
\end{tabular}
\caption{Heart-rate Dataset Split}
\label{table:hear_rate_split}
\end{table}

Regarding the parameters of the rolling-window, we set the length of the window to 32 or 8 seconds of samples, following the authors in \cite{reiss2019deep}. Regarding the step-size, it was decided to choose this number so that the auto-correlation around the lag 2000 is 0.6 (see figure \ref{fig:acorr_hr}). This decision is arbitrary, but it is a compromise, as bigger numbers would result in less available virtual tasks. The step-size was set accordingly to be 4.


\begin{figure} [H]
\centering
\includegraphics[width=6cm]{supplementary-images/acorr_hr.pdf}
\caption{Auto-correlation of the target in Heart-rate Dataset.}
\label{fig:acorr_hr}
\end{figure}

\subsection{Battery Dataset Pre-processing}

We do not provide any further information on BATTERY dataset since this is private data.


\section{Interpretation of MAML for TSR}
Now, we want to present a reformulation of the loss in equation 2 in the main paper, which may shed light on an interpretation of the representation learned by MAML. Assuming that we have only a virtual task (two contiguous meta-windows) and our loss is MAE, we simplify the aforementioned equation as:

\begin{equation}
\min_{ \theta }  \sum_{{ (\mathbf{x}_j, \mathbf{y}_j) \in \mathcal{T}_{t+1}  }} ||\mathbf{y}_j - f_{ \theta-\alpha \nabla_{ \theta}\mathcal{L}_{\mathcal{T}_{t}}(f_{ \theta})}(\mathbf{x}_j)  ||_1
\label{eq:inter_1}
\end{equation}
Particularly, we will assume $f_{\theta}$ denotes a model that transforms linearly the output of a feature extractor $\phi(x_j)$ such that:

\begin{equation}
f_{\theta}(\mathbf{x}_j) =  \theta^T \phi(\mathbf{x}_j)
\label{eq:inter_2}
\end{equation}
Therefore, we can express the loss in the inner loop (lower index in equation \ref{eq:inter_2}) as:

\begin{equation}
\mathcal{L}_{\mathcal{T}_t} (f_{\theta}) =  \sum_{{ (\mathbf{x}_i, \mathbf{y}_i) \in \mathcal{T}_{t}  }} ||\mathbf{y}_i - f_{\theta}(\mathbf{x}_i)||_1 = \sum_{{ (\mathbf{x}_i ,\mathbf{y}_i) \in \mathcal{T}_{t}  }} ||\mathbf{y}_i - \theta^T \phi(\mathbf{x}_i)||_1
\label{eq:inter_3}
\end{equation}
And the gradient of this loss is given by:

\begin{equation}
\nabla_{\theta} \mathcal{L}_{\mathcal{T}_t} (f_{\theta})  = -\sum_{{ (\mathbf{x}^{(t)}_i, \mathbf{y}^{(t)}_i) \in \mathcal{T}_{t}  }} \mathrm{sign}( \mathbf{y}^{(t)}_i - {\theta}^T\phi(\mathbf{x}^{(t)}_i))  \cdot \phi(\mathbf{x}^{(t)}_i)  = \Delta^{(t)}
\label{eq:inter_4}
\end{equation}

Where we have included the \textbf{upper index} to denote the time-step of the meta-window to whom the samples belong. Moreover, using the equation \ref{eq:inter_2} and \ref{eq:inter_4}, we reformulate the equation \ref{eq:inter_1} as:

\begin{equation}
\begin{split}
\min_{ \theta }  \sum_{{ (\mathbf{x}_j, \mathbf{y}_j) \in \mathcal{T}_{t+1}  }} ||\mathbf{y}^{(t+1)}_j -  (\theta-\alpha \Delta^{(t)})^T\phi(\mathbf{x}^{(t+1)}_j)  ||_1 \\=  \sum_{{ (\mathbf{x}_j, \mathbf{y}_j) \in \mathcal{T}_{t+1}  }} ||\mathbf{y}^{(t+1)}_j -  (\theta^T\phi(\mathbf{x}^{(t+1)}_j) -\alpha (\Delta^{(t)})^T \phi(\mathbf{x}^{(t+1)}_j))  ||_1  \\
= \sum_{{ (\mathbf{x}_j, \mathbf{y}_j) \in \mathcal{T}_{t+1}  }} ||\mathbf{y}^{(t+1)}_j -  (\theta^T\phi(\mathbf{x}^{(t+1)}_j) -\epsilon _j )||_1 
\label{eq:inter_5}
\end{split}\end{equation}

We can interpret $\epsilon_j = \alpha (\Delta^{(t)})^T \phi(\mathbf{x}^{(t+1)}_j)$ as a \textbf{correcting factor} that aims to reduce the error in the prediction on the new meta-window $\mathcal{T}_{t+1}$ by using the previous meta-window $\mathcal{T}_t$. Furthermore, this correcting factor can be expressed as:

\begin{equation}
\begin{split} \epsilon_j =
 (\Delta^{(t)})^T \phi(\mathbf{x}^{(t+1)}_j) =    -  \left(\sum_{{ (\mathbf{x}^{(t)}_i, \mathbf{y}^{(t)}_i) \in \mathcal{T}_{t}  }} \mathrm{sign}( \mathbf{y}^{(t)}_i - {\theta}^T\phi(\mathbf{x}^{(t)}_i))  \cdot \phi(\mathbf{x}^{(t)}_i) \right)^T \phi(\mathbf{x}^{(t+1)}_j)
  \\
  = -  \sum_{{ (\mathbf{x}^{(t)}_i, \mathbf{y}^{(t)}_i) \in \mathcal{T}_{t}  }} \mathrm{sign}( \mathbf{y}^{(t)}_i - {\theta}^T\phi(\mathbf{x}^{(t)}_i) )\cdot \phi(\mathbf{x}^{(t)}_i) ^T \phi(\mathbf{x}^{(t+1)}_j)
\end{split}
\label{eq:inter_6}
\end{equation}
By denoting $\mathrm{err}(\mathbf{x}^{(t)}_i, \mathbf{y}^{(t)}_i) = \mathrm{sign}( \mathbf{y}^{(t)}_i - {\theta}^T\phi(\mathbf{x}^{(t)}_i) )$ and reinterpreting $\phi(\mathbf{x}^{(t)}_i) ^T \phi(\mathbf{x}^{(t+1)}_j)$ as a kernel $\kappa(\mathbf{x}^{(t)}_i, \mathbf{x}^{(t+1)}_j)$, we rewrite the equation \ref{eq:inter_6} as:


\begin{equation}
\epsilon_j = -  \sum_{{ (\mathbf{x}^{(t)}_i, \mathbf{y}^{(t)}_i) \in \mathcal{T}_{t}  }} \mathrm{err}(\mathbf{x}^{(t)}_i, \mathbf{y}^{(t)}_i) \cdot  \kappa(\mathbf{x}^{(t)}_i, \mathbf{x}^{(t+1)}_j)
\end{equation}
The equation \ref{eq:inter_6}, therefore, shows that the correcting factor $\epsilon$ takes into account the error of the support set and corrects the predictions on the query set proportionally to a kernel between the query and the support set. If  $\kappa(\mathbf{x}^{(t)}_i,\mathbf{x}^{(t+1)}_j) > 0$, then we can further interpret the kernel as a similarity between the element of the query set and the element of the support set. Given our setting and the mentioned assumptions, it is possible to see that the loss function in equation 2 finds a metric space (or embedding space) that allows a prediction to be corrected by accounting immediately previous temporal data.
Interestingly, in case some other task loss ($\mathcal{L}_{\mathcal{T}}$) is used, the interpretation does not change too much. For instance, if MSE is used, it implies to set $\mathrm{err}(\mathbf{x}^{(t)}_i, \mathbf{y}^{(t)}_i) = \mathbf{y}^{(t)}_i - {\theta}^T\phi(\mathbf{x}^{(t)}_i) $.

The update rule learnt through MAML for TSR $\theta^{(t)}=\theta-\alpha \Delta^{(t)} $ is somewhat related to the update rule in \textbf{recursive least squares} (RLS) algorithm \cite{hayes2009statistical} \cite{murphy2012machine} $\theta^{(t)}=\theta^{(t-1)}+K^{(t)} \mathrm{err}(\mathbf{x}^{(t)}, \mathbf{y}^{(t)})$, where $K^{(t)}$ is the kalman gain. Both of them compute an \textbf{online update} for the parameters which includes a measure of the error. The difference is, however, that the update in RLS is on temporally previous parameters ($\theta^{(t-1)}$), while MAML is on fixed time-independent parameters $\theta$. It is, therefore, possible to use MAML for TSR as an \textbf{online parameter learning algorithm} for TSR.


\section{Embeddings of meta-windows and embeddings of updated parameters}

After training the models, we explore the encodings of the meta-windows by plotting the T-SNE embeddings. The figure \ref{fig:task_embeddings} shows the results, where every point is a meta-window and the color is an indicator of the original very-long time series used to create the meta-windows. It is noticeable that the meta-windows coming from the same time series (same color) are creating clusters. 

Moreover, we also plot the T-SNE embeddings of the updated parameters. It means, the parameters that we obtain after selecting a given meta-window and running a gradient update on the parameters of the last layer. The embeddings for the updates using MAML and simple fine-tuning on Resnet are shown in figure \ref{fig:resnet_parameter_embeddings_pollution}, where is possible to see that the parameters updated by MAML exhibit more strcuture and are distributed around the initial value (red dot).

\begin{figure}[H]
\centering
\vspace{-2\baselineskip}
\subfloat[Resnet, TRAIN]{\label{fig:topleft}{\includegraphics[width=0.45\textwidth]{supplementary-images/POLLUTION-RESNET-TRAIN.pdf}}}\hfill
\subfloat[MAML, Train]{\label{fig:topleft}{\includegraphics[width=0.45\textwidth]{supplementary-images/POLLUTION-MAML-TRAIN.pdf}}}\hfill

\subfloat[Resnet, Validation]{\label{fig:topright}{\includegraphics[width=0.45\textwidth]{supplementary-images/POLLUTION-RESNET-VALIDATION.pdf}}} \hfill
\subfloat[MAML, Validation]{\label{fig:topleft}{\includegraphics[width=0.45\textwidth]{supplementary-images/POLLUTION-MAML-VALIDATION.pdf}}}\hfill

\subfloat[Resnet, Test]{\label{fig:mdleft}{\includegraphics[width=0.45\textwidth]{supplementary-images/POLLUTION-RESNET-TEST.pdf}}}\hfill
\subfloat[MAML, Test]{\label{fig:topleft}{\includegraphics[width=0.45\textwidth]{supplementary-images/POLLUTION-MAML-TEST.pdf}}}\hfill

\subfloat[Resnet, All Datasets]{\label{fig:mdleft}{\includegraphics[width=0.45\textwidth]{supplementary-images/POLLUTION-RESNET-ALL.pdf}}}\hfill
\subfloat[MAML, All Datasets]{\label{fig:topleft}{\includegraphics[width=0.45\textwidth]{supplementary-images/POLLUTION-ALL-DATASETS.pdf}}}\hfill
\caption{Embeddings of updated parameters  for POLLUTION (Resnet and MAML).}
\label{fig:resnet_parameter_embeddings_pollution}
\end{figure}


\begin{figure}[H]
\centering
\subfloat[]{\label{fig:topleft}{\includegraphics[width=0.33\textwidth]{supplementary-images/POLLUTION_Meta-window_Embeddings.pdf}}}\hfill
\subfloat[]{\label{fig:topright}{\includegraphics[width=0.33\textwidth]{supplementary-images/HR_Meta-window_Embeddings.pdf}}}
\subfloat[]{\label{fig:mdleft}{\includegraphics[width=0.33\textwidth]{supplementary-images/BATTERY_Meta-window_Embeddings.pdf}}}\hfill

\caption{Virtual task embeddings computed with T-SNE from the encoder output ($l$ = 50).}
\label{fig:task_embeddings}
\end{figure}


\subsection{Similarity between dataset splits}

Measuring the task similarity is beyond the scope of this thesis, however, assessing the similarity between the dataset splits (train, test and validation), may provide useful insights to draw conclusions about the results.  To measure the similarity between those splits, we use the distance between the mean of the task embeddings ($z$ in our formulation). Through this method, the tables \ref{table:similarity_50} show that the splits test and validation are very similar to each other in BATTERY, by comparing to the similarity between train-validation. Later on, we will provide an analysis to explain how this fact affected the results.


\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{COMPARISON} & \textbf{POLLUTION} & \textbf{HR} & \textbf{BATTERY} \\ \hline
\textbf{Train-Test} & 0.2886            & 0.2524      & 0.0775           \\ \hline
\textbf{Train-Validation}  & 0.3056             & 0.2368      & 0.0814           \\ \hline
\textbf{Test-Validation}   & 0.2987             & 0.1738      & 0.0150           \\ \hline
\end{tabular}
\caption{Similarity between meta-datasets (meta-windows with $l$=50).}
\label{table:similarity_50}
\end{table}






\section{Hyper-parameter Tuning}

The following tables present the final hyper-parameters used for each approach after performing the grid search.

\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{Model} & \textbf{Steps} & \textbf{\begin{tabular}[c]{@{}c@{}}Fine-tuning \\ LR\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Weight \\ Decay\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Training \\ LR\end{tabular}} \\ \hline
POLLUTION        & RESNET         & 1              & 0.001                                                              & 0.001                                                            & 0.01                                                            \\ \hline
POLLUTION        & RESNET         & 10             & 0.001                                                              & 0.001                                                            & 0.01                                                            \\ \hline
HR               & RESNET         & 1              & 0.001                                                              & 0.01                                                             & 0.0001                                                          \\ \hline
HR               & RESNET         & 10             & 0.001                                                              & 0                                                                & 0.0001                                                          \\ \hline
BATTERY          & RESNET         & 1              & 0.001                                                              & 0                                                                & 0.01                                                            \\ \hline
BATTERY          & RESNET         & 10             & 0.001                                                              & 0.01                                                             & 0.01                                                            \\ \hline
POLLUTION        & VRADA         & 1              & 0.0001                                                             & 0.01                                                             & 0.0003                                                          \\ \hline
POLLUTION        & VRADA         & 10             & 0.0001                                                             & 0.01                                                             & 0.0003                                                          \\ \hline
HR               & VRADA         & 1              & 0.001                                                              & 0                                                                & 0.0003                                                          \\ \hline
HR               & VRADA         & 10             & 0.001                                                              & 0.01                                                             & 0.0003                                                          \\ \hline
BATTERY          & VRADA         & 1              & 0.0001                                                             & 0                                                                & 0.0003                                                          \\ \hline
BATTERY          & VRADA         & 10             & 0.0001                                                             & 0                                                                & 0.0003                                                          \\ \hline
POLLUTION        & LSTM           & 1              & 0.01                                                               & 0.5                                                              & 0.00001                                                         \\ \hline
POLLUTION        & LSTM           & 10             & 0.001                                                              & 0.5                                                              & 0.00001                                                         \\ \hline
HR               & LSTM           & 1              & 0.01                                                               & 0                                                                & 0.0001                                                          \\ \hline
HR               & LSTM           & 10             & 0.01                                                               & 0.1                                                              & 0.0001                                                          \\ \hline
BATTERY          & LSTM           & 1              & 0.001                                                              & 0.5                                                              & 0.0001                                                          \\ \hline
BATTERY          & LSTM           & 10             & 0.001                                                              & 0.01                                                             & 0.0001                                                          \\ \hline
\end{tabular}
\caption{Baselines Set-up ($l$=50)}
\label{table:baselines_setup}
\end{table}



\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{Model} & \textbf{Steps}  & \textbf{Meta-LR} & \textbf{LR} & \shortstack{\textbf{Noise } \\ \textbf{Level}} &  \shortstack{\textbf{VRAE} \\ \textbf{Weight}}\\ \hline
POLLUTION        & MAML           & 1                         & 0.0005                        & 0.01                   & 0.01                 & -                    \\ \hline
POLLUTION        & MAML           & 10                        & 0.0005                        & 0.001                  & 0.01                 & -                    \\ \hline
POLLUTION        & MMAML          & 1                         & 0.0005                        & 0.01                   & 0.001                & 0.1                  \\ \hline
POLLUTION        & MMAML          & 10                        & 0.0005                        & 0.001                  & 0.001                & 0.1                  \\ \hline
HR               & MAML           & 1                         & 0.0005                        & 0.01                   & 0.01                 & -                    \\ \hline
HR               & MAML           & 10                        & 0.0005                        & 0.01                   & 0.01                 & -                    \\ \hline
HR               & MMAML          & 1                         & 0.0005                        & 0.01                   & 0.01                 & 0.01                 \\ \hline
HR               & MMAML          & 10                        & 0.0005                        & 0.01                   & 0.01                 & 0.01                 \\ \hline
BATTERY          & MAML           & 1                         & 0.00005                       & 0.0001                 & 0                    & -                    \\ \hline
BATTERY          & MAML           & 10                        & 0.00005                       & 0.0001                 & 0                    & -                    \\ \hline
BATTERY          & MMAML          & 1                         & 0.00005                       & 0.0001                 & 0                    & 0.0001               \\ \hline
BATTERY          & MMAML          & 10                        & 0.00005                       & 0.0001                 & 0                    & 0.0001               \\ \hline
\end{tabular}
\caption{MAML and MMAML Setup ($l$=50)}
\label{table:maml_setup}

\end{table}



\end{document}



